Cerberus: A Formal Approach to Secure and Efficient Enclave Memory Sharing

Hardware enclaves rely on a disjoint memory model, which maps each physical address to an enclave to achieve strong memory isolation. However, this severely limits the performance and programmability of enclave programs. While some prior work proposes enclave memory sharing, it does not provide a formal model or verification of their designs. This paper presents Cerberus, a formal approach to secure and efficient enclave memory sharing. To reduce the burden of formal verification, we compare different sharing models and choose a simple yet powerful sharing model. Based on the sharing model, Cerberus extends an enclave platform such that enclave memory can be made immutable and shareable across multiple enclaves via additional operations. We use incremental verification starting with an existing formal model called the Trusted Abstract Platform (TAP). Using our extended TAP model, we formally verify that Cerberus does not break or weaken the security guarantees of the enclaves despite allowing memory sharing. More specifically, we prove the Secure Remote Execution (SRE) property on our formal model. Finally, the paper shows the feasibility of Cerberus by implementing it in an existing enclave platform, RISC-V Keystone.

==> makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

FIGURES = # mssa_comparison*.pdf

PDF = main.pdf

startdocker:
	docker run -v `pwd`:/home/latex --rm --name=latexrun -it aergus/latex /bin/bash

ifeq ($(LATEX_BUILD_ENV),docker)
docker: *.tex *.bib
	docker run -v `pwd`:/home/latex --rm --name=latexrun -it aergus/latex /bin/bash -c "cd home/latex;make"
else

all:  ${PDF}

diff:
	git-latexdiff -b --main main.tex 57745d11adf70f777a4a094a636f839d112886bb

# %.tex needed as it create the first element used by special $ sequences below
%.pdf:  %.tex *.tex *.bib $(FIGURES)
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

endif

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.fls *.fdb_latexmk

clean: docclean
	$(RM)  $(PACKAGE).cls \=

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

.PHONY: all  docclean clean distclean


==> response_letter.tex <==
\newpage
\clearpage
\section*{Response Letter for Revision}

This paper was submitted to the second cycle of ACM CCS 2022 and received a \textit{Revision} decision. Since then, we have worked to improve the writing of the submission, demonstrated the practicality of our sharing model using our case studies, clarified ambiguities on limitations and formalisms, and updated the artifacts. We have done our best to address all the comments of the reviewers. We thank the reviewers for their insightful feedback on the previous version, which helped us improve the submission.

We first address the required changes for the revision decision from the concerns and then discuss the additional changes we made to the paper.

\subsection{\textbf{Required Changes}}

\subsubsection{\textbf{Practicality of Our Sharing Model}}

\begin{quote}
\it Reviewer 1: Demonstrate the proposed sharing model is the practically useful by using case studies mentioned in the response. (no new case studies need to be implemented, though it would be a plus)
\end{quote}
\begin{quote}
\it 
Reviewer 2: Consider bringing forward supported applications/performance speedup of single-shared abstraction.
\end{quote}

We have introduced the use cases of memory sharing in \S\ref{sec:use_cases_of_sharing},  focusing on the single-sharing model.
We also incorporated the text from our rebuttal response to discuss performance comparison with previous work in \S\ref{sec:discussion}.



\subsubsection{\textbf{Limitations}}
\begin{quote}
\it Reviewer 1: Round out the discussions on limitations by incorporating texts from the response.
\end{quote}

\S\ref{sec:writable_shared_memory} clarifies that \cerberus does not focus on writable shared memory with dynamic permissions and that \cerberus shares the same limitation as PIE~\cite{pie} in terms of supported applications.
Next, \S\ref{sec:single_sharing} and Figure~\ref{fig:capped_vs_single} compare the capped- and single-sharing models and clarify the limitation of the single-sharing model.
Finally, \S\ref{sec:assumptions} clarifies the limitations of the \tapc model by adding to the list of assumptions.
The clarification includes stating each of the limitations that the \tapc model inherits from the \tap model.

\subsubsection{\textbf{Formalism Ambiguities}}
\label{rl:formal_ambiguities}

\begin{quote}
\it Reviewer 1:Improve the formal sections: clarify the noninterference definition, clean up the formal definitions so variables are properly quantified.
\end{quote}
We improved the formal development of our work by first clarifying the non-interference definition in \S\ref{sec:guarantees}. We state the differences between our observational determinism-based properties with typical non-interference and reference prior work that initially defines observational determinism. We also provide references to existing work that uses the observational determinism-based definitions of integrity and confidentiality.

\begin{quote}
\it Reviewer 2: Clarify formal/notational ambiguities outlined above.
\end{quote}
We also made the following changes to address the formal ambiguities:
\begin{itemize}
    \item Explicitly included the domains of all the quantifiers in \S\ref{sec:guarantees}
    \item Fixed the spacing for logical connectives in the formulas in \S\ref{sec:new_ops} and \S\ref{sec:guarantees}
    \item Defined the set of variable $V$ in Table~\ref{fig:tap_c_state_vars}
    \item Reordered conjucts of formulas with their descriptions so they are presented in the same order in \S\ref{sec:new_ops}
    \item Fixed Eq.~\ref{eq:clone_success_cond} so that the the current executing process is the operating system and the parent is required to be a valid enclave
\end{itemize}

\begin{quote}
\it Reviewer 2: Clone takes the child ID as an argument, but how does the OS select this ID? What if an enclave with this ID already exists?
\end{quote}
Lastly, we fixed Eq.~\ref{eq:clone_success_cond} so that the condition conforms to formal models, which checks that the given child ID is not pointing to an \textit{active} enclave but it is a \textit{valid} enclave ID. We introduced the \textit{active} predicate to indicate when an enclave is launched and not destroyed and a \textit{valid} predicate to indicate if the ID is a valid enclave ID. This notation very closely matches the formal models up besides naming.

\subsubsection{\textbf{Artifact Update}}

\begin{quote}
	\it Reviewer 1: Provide a link to the artifact.
\end{quote}
We have added the artifact to our anonymous Github repository \url{https://github.com/anonymous1721/TAPC}.

\subsection{\textbf{Additional Changes}}

\subsubsection{\textbf{Definition of SRE and Decomposition Theorem}}

\begin{quote}
\it Reviewer 3: The main goal is to formally prove that $TAP_C$ satisfies the SRE property, but no formal definition of the SRE property is given.
\end{quote}

\begin{quote}
\it Reviewer 3: In Section 5, the reference to Theorem 3.2 [50] is used to state that the triad of properties later defined are sufficient for SRE, but the theorem is not stated, not even its hypothesis is given, and the reader still does not know what the formal definition of SRE is.
\end{quote}

We have also stated the definition of \sre and the decomposition theorem from prior work for ease of reference.

\subsubsection{\textbf{Additional Changes to Formal Development}}

\begin{quote}
\it Reviewer 3: In Section 4.5, Security Arguments are given for the new Clone and Snapshot operations. But it is not clear whether these arguments are informal statements of something that is to be formally proved later or whether they are informal statements of something that will be built upon later.
\end{quote}


\begin{quote}
\it Reviewer 3: The footnotes explaining standard notation (element of, maps, singleton sets, union) are superfluous and in some cases confusing, for example, the star symbol next to the set S on page 5.
\end{quote}

In addition to \S\ref{rl:formal_ambiguities}, we have also made the following changes to improve the formal development:
\begin{itemize}
    \item Removed the informal justifications of the proofs and refer the reader to the formal models in the artifact
    \item Removed all superfluous explanations of common notation and add these to the \S\ref{appendix}
\end{itemize}

